Parsing Natural Language Sentences by Semi-supervised Methods

We present our work on semi-supervised parsing of natural language sentences, focusing on multi-source crosslingual transfer of delexicalized dependency parsers. We first evaluate the influence of treebank annotation styles on parsing performance, focusing on adposition attachment style. Then, we present KLcpos3, an empirical language similarity measure, designed and tuned for source parser weighting in multi-source delexicalized parser transfer. And finally, we introduce a novel resource combination method, based on interpolation of trained parser models.

==> results.tex <==
% OUTPUT
bn & Bengali & 1 & $^L$\np{49.50738916} & 61.0 & 74.1 & te & 66.7 & 0.5 & \textbf{te} & 66.7 & 63.2 & 66.7 & \textbf{\np{67.1182266}} & 66.9 \\
cs & Czech & 174 & $^L$\np{26.11040061} & 60.5 & 68.1 & sk & \textbf{\np{65.8261611}} & 0.3 & \textbf{sk} & \textbf{\np{65.8261611}} & 60.4 & \textbf{\np{65.8261611}} & 57.5 & 65.2 \\
da & Danish & 6 & $^L$\np{25.08544087} & 56.2 & 71.0 & en & \textbf{\np{55.43403964}} & 0.5 & sl & 42.1 & \textbf{\np{54.4429255}} & 50.3 & 48.9 & 49.5 \\
\hdashline
de & German & 32 & $^L$\np{31.40823526} & 12.6 & 76.4 & en & 56.8 & 0.7 & \textbf{en} & 56.8 & 27.6 & 56.8 & 18.2 & \textbf{\np{61.6083414}} \\
en & English & 5 & $^L$\np{27.38356986} & 12.3 & 70.5 & de & 42.6 & 0.8 & \textbf{de} & 42.6 & 21.1 & 42.6 & 16.2 & \textbf{\np{48.59084549}} \\
eu & Basque & 14 & $^R$\np{22.03864464} & 41.2 & 65.3 & da & \textbf{\np{42.06104733}} & 0.7 & tr & 29.1 & \textbf{\np{40.78689443}} & 30.6 & 39.5 & 34.9 \\
\hdashline
gr & Anc. Greek & 6 & $^L$\np{18.49050261} & 43.2 & 50.6 & et & 42.2 & 1.0 & sl & 34.0 & \textbf{\np{44.74701631}} & 42.6 & 41.4 & 44.0 \\
la & Latin & 5 & $^L$\np{18.27103779} & 38.1 & 42.8 & gr & 40.3 & 1.2 & cs & 35.0 & \textbf{\np{40.32157027}} & 39.7 & 39.7 & 39.5 \\
nl & Dutch & 6 & $^L$\np{26.53536258} & 55.0 & 67.0 & da & 57.9 & 0.7 & \textbf{da} & 57.9 & 56.2 & 58.7 & 54.2 & \textbf{\np{59.3912265}} \\
\hdashline
pt & Portuguese & 6 & $^L$\np{27.64615647} & 62.8 & 74.1 & en & 64.2 & 0.2 & es & 62.7 & \textbf{\np{67.15527527}} & 62.7 & 62.8 & 63.7 \\
ro & Romanian & 3 & $^L$\np{32.1969697} & 44.2 & 81.7 & it & \textbf{\np{66.36363636}} & 1.6 & la & 30.8 & \textbf{\np{51.21212121}} & 50.0 & 48.6 & 50.3 \\
ru & Russian & 3 & $^L$\np{32.59109312} & 55.5 & 67.3 & sk & 57.7 & 0.9 & la & 40.4 & \textbf{\np{57.80798149}} & 57.2 & 53.3 & 56.3 \\
\hdashline
sk & Slovak & 86 & $^L$\np{24.59615049} & 52.2 & 68.3 & cs & \textbf{\np{61.65377682}} & 0.2 & sl & 58.4 & 59.6 & 58.4 & 55.7 & \textbf{\np{60.58382276}} \\
sl & Slovenian & 6 & $^L$\np{22.67605634} & 45.9 & 63.6 & sk & \textbf{\np{53.86541471}} & 0.2 & \textbf{sk} & \textbf{\np{53.86541471}} & 47.1 & \textbf{\np{53.86541471}} & 42.8 & 49.6 \\
sv & Swedish & 6 & $^L$\np{26.90947666} & 45.4 & 78.1 & de & \textbf{\np{61.61598303}} & 0.6 & da & 49.8 & \textbf{\np{52.29844413}} & 50.8 & 49.4 & 50.4 \\
\hdashline
ta & Tamil & 2 & $^L$\np{33.93665158} & 27.85 & 66.3 & hi & \textbf{\np{53.54449472}} & 1.1 & tr & 31.1 & 28.0 & \textbf{\np{39.96983409}} & 27.6 & 37.3 \\
te & Telugu & 1 & $^L$\np{59.12897822} & 67.8 & 77.4 & bn & \textbf{\np{77.38693467}} & 0.4 & \textbf{bn} & \textbf{\np{77.38693467}} & 68.7 & \textbf{\np{77.38693467}} & 72.9 & \textbf{\np{77.38693467}} \\
tr & Turkish & 5 & $^L$\np{36.58320408} & 18.8 & 71.2 & ta & 40.3 & 0.7 & \textbf{ta} & 40.3 & 23.2 & \textbf{\np{41.05916242}} & 25.3 & 34.8 \\
\hline
\multicolumn{2}{|l}{\textbf{Average on test}}  & 20 & 30.1 & 44.5 & 68.5 &  & \textbf{\np{55.9110837}} & 0.7 & \textbf{} & 48.6 & 48.0 & 52.5 & 45.6 & \textbf{\np{52.76828271}} \\
\hdashline
\multicolumn{2}{|l}{\textbf{Std. dev. on test}} &  & 10.3 & 16.9 & 9.4 &  & 10.8 &  & \textbf{} & 14.4 & 15.0 & 11.8 & 16.0 & 12.0 \\
\hline
\hline
ar & Arabic & 28 & $^R$\np{34.20551342} & 37.3 & 67.1 & ro & \textbf{\np{43.05430759}} & 1.7 & sk & 41.2 & 35.3 & \textbf{\np{41.3363045}} & 30.7 & 34.6 \\
bg & Bulgarian & 6 & $^L$\np{27.1991911} & 63.9 & 74.8 & sk & 66.8 & 0.4 & \textbf{sk} & 66.8 & 66.0 & 67.4 & 60.3 & \textbf{\np{68.45298281}} \\
ca & Catalan & 53 & $^L$\np{29.5784212} & 56.3 & 73.6 & es & 72.4 & 0.1 & \textbf{es} & 72.4 & 61.5 & 72.4 & 58.5 & \textbf{\np{72.37008394}} \\
\hdashline
el & Greek & 5 & $^L$\np{31.4113239} & 63.1 & 71.1 & sk & 61.4 & 0.7 & cs & 60.7 & 62.3 & 63.8 & 59.6 & \textbf{\np{64.13405495}} \\
es & Spanish & 50 & $^L$\np{28.75238247} & 60.0 & 73.8 & ca & 72.7 & 0.0 & \textbf{ca} & 72.7 & 64.3 & 72.7 & 60.4 & \textbf{\np{72.74857052}} \\
et & Estonian & 1 & $^L$\np{24.16317992} & 67.8 & 79.8 & hu & 71.8 & 0.9 & da & 64.9 & 70.5 & \textbf{\np{71.9665272}} & 67.4 & 71.7 \\
\hdashline
fa & Persian & 7 & $^R$\np{28.99611592} & 32.0 & 59.2 & ar & \textbf{\np{35.64386017}} & 1.1 & cs & \textbf{\np{34.70271885}} & 32.5 & 33.3 & 29.5 & 28.6 \\
fi & Finnish & 5 & $^L$\np{33.5483871} & 40.8 & 55.4 & et & 44.2 & 1.1 & \textbf{et} & 44.2 & 41.7 & \textbf{\np{47.13364055}} & 41.5 & 44.7 \\
hi & Hindi & 26 & $^R$\np{26.73758328} & 27.2 & 76.1 & ta & \textbf{\np{56.26135675}} & 1.1 & fa & 20.8 & 24.6 & 27.2 & 26.2 & \textbf{\np{32.74152029}} \\
\hdashline
hu & Hungarian & 7 & $^L$\np{32.28485839} & 55.65 & 67.5 & et & 52.0 & 0.7 & cs & 46.0 & 56.5 & 51.2 & \textbf{\np{57.39379085}} & 53.0 \\
it & Italian & 5 & $^L$\np{31.53453689} & 54.81 & 71.6 & ca & 59.8 & 0.3 & pt & 54.9 & 59.5 & 59.6 & 56.0 & \textbf{\np{60.10596546}} \\
ja & Japanese & 6 & $^R$\np{39.48520399} & 32.11 & 81.9 & tr & \textbf{\np{49.23831203}} & 2.2 & ta & \textbf{\np{44.86079496}} & 28.8 & 34.1 & 27.2 & 33.0 \\
\hline
\multicolumn{2}{|l}{\textbf{Average on dev}}  & 17 & 30.7 & 49.3 & 71.0 &  & \textbf{\np{57.10675971}} & 0.9 & \textbf{} & 52.0 & 50.3 & \textbf{\np{53.51649087}} & 47.9 & 53.0 \\
\hdashline
\multicolumn{2}{|l}{\textbf{Std. dev. on dev}} &  & 4.0 & 14.4 & 7.8 &  & 12.5 &  & \textbf{} & 16.1 & 16.5 & 16.7 & 15.6 & 17.4 \\
\hline
\hline
\multicolumn{2}{|l}{\textbf{Average on all}}  & 19 & 30.3 & 46.4 & 69.5 &  & \textbf{\np{56.38935411}} & 0.8 & \textbf{} & 50.0 & 48.9 & \textbf{\np{52.91575378}} & 46.5 & 52.9 \\
\hdashline
\multicolumn{2}{|l}{\textbf{Std. dev. on all}} &  & 8.2 & 15.9 & 8.7 &  & 11.3 &  & \textbf{} & 15.0 & 15.4 & 13.7 & 15.6 & 14.1 \\

